Extracurricular Learning: Knowledge Transfer Beyond Empirical Distribution

Knowledge distillation has been used to transfer knowledge learned by a sophisticated model (teacher) to a simpler model (student). This technique is widely used to compress model complexity. However, in most applications the compressed student model suffers from an accuracy gap with its teacher. We propose extracurricular learning, a novel knowledge distillation method, that bridges this gap by (1) modeling student and teacher output distributions; (2) sampling examples from an approximation to the underlying data distribution; and (3) matching student and teacher output distributions over this extended set including uncertain samples. We conduct rigorous evaluations on regression and classification tasks and show that compared to the standard knowledge distillation, extracurricular learning reduces the gap by 46% to 68%. This leads to major accuracy improvements compared to the empirical risk minimization-based training for various recent neural network architectures: 16% regression error reduction on the MPIIGaze dataset, +3.4% to +9.1% improvement in top-1 classification accuracy on the CIFAR100 dataset, and +2.9% top-1 improvement on the ImageNet dataset.

==> rebuttal.tex <==
% \documentclass{article}

% \usepackage{neurips_2020_author_response}

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{graphicx}
% \usepackage{lipsum}

% \begin{document}

\section{Rebuttal}


{\bf R1:}

We thank the reviewer for pointing us to a relevant recent paper (Wang et al. 2020), which uses MixUp for a different goal. We will mention their approach in our modified paper. Please see response to R3 for the question on novelty.

{\bf R3:} 

We thank the reviewer for pointing us to great works on distillation with uncertainty estimation. These works can be used to improve uncertainty estimation in XCL to further reduce the gap. We will cover them in the paper.

% \end{document}


==> uncertainty_ablation.tex <==
\subsection{Observations}\label{sec:observe}
\new{In this section, we discuss two set of experiments for classification tasks to investigate the role of i) sampling uncertain data, and ii) transferring additional information through uncertainly estimation, to improve KD.}

% \subsection{Uncertainty Ablation}\label{sec:evidence}

% \new{In this section, we validate the hypothesis that high uncertainty points in the empirical input distribution are more effective for matching the student predictions with those of the teacher. The intuition is that uncertain data points are located on the decision boundaries in the teacher model. By fitting the student to such data points, we encourage the decision boundaries of the student to imitate those of the teacher, therefore, helping with transferring generalization properties of the teacher to the student. We devise a comprehensive set of ablation studies to investigate the role of training data uncertainty on student generalization accuracy in classification tasks. Our experiments utilize various data distributions and target two main sources of uncertainty, namely, aleatoric and distribution uncertainty.}

\noindent\textbf{Observation 1 (Aleatoric Uncertainty).} 
\new{
Here, we target aleatoric uncertainty, which refers to the inherent confusing features of a sample, and show its role in KD. We randomly divide the data available in the training set into two disjoint subsets represented by $\mathcal{S}$ and $\mathcal{U}$. $\mathcal{S}$ corresponds to half of the data that is seen during the training of the teacher while $\mathcal{U}$ denotes a held-out set. In this setting, the per-class images are balanced across all data subsets. Once the teacher is trained using data in $\mathcal{S}$, we leverage the entropy of softmax predictions generated by the teacher to sort samples in $\mathcal{U}$. We then split $\mathcal{U}$ into two equally sized distjoint subsets $\mathcal{U} = \mathcal{H} \cup \mathcal{L}$, corresponding to samples with high and low uncertainties, respectively. 
% as shown in Figure~\ref{fig:data_subsets}.
% quantify uncertainty on data samples. 
%Generally, due to overfitting, the teacher is over-confident on the training set, resulting in a close to zero uncertainty on \textit{S}. 
% Using the trained teachers and our measure of uncertainty, we further divide the remaining data in \textit{U} into two equally sized subsets, dubbed \textit{H} and \textit{L}, corresponding to high and low uncertainties, respectively. Figure~\ref{fig:data_subsets} illustrates the dataset division.
}

% \begin{SCfigure}[50][h]
%     \centering
%     \resizebox{0.5\columnwidth}{!}{
%     \includegraphics{figures/Piechart.png}
%     \caption{\new{Dataset division for isolating the effect of aleatoric uncertainty on KD generalization accuracy.}}
%     \label{fig:data_subsets}}
% \end{SCfigure}

%For CIFAR100, the student is a ResNet-18 and the teachers are an ensemble of 8 ResNet-18 models trained on \textit{S} with a top-1 validation accuracy of $74.7\%$. 
% Both the student and the teachers are trained for 400 epochs. 
%For ImageNet, the student is a ResNet-50 and the teachers are an ensemble of 4 ResNet-50 models trained on \textit{S} with a top-1 validation accuracy of $76.1\%$.

\new{For a soft-label $y$ we define its normalized entropy as}
\begin{equation}
 \hat{H}(y) = -\sum_{j=1}^c y^j \log y^j / \log c,   
\end{equation}
\new{where superscript $j$ refers to the $j$'th component of the vector, and $c$ is the number of classes. $\hat{H}(y)$ varies between $0$ and $1$, and denotes label uncertainty for a sample. It can also be interpreted as the amount of additional information encoded in soft labels compared to one-hot labels.}

\new{Table~\ref{tab:aleatoric} encloses the results for training a student on each of the above-mentioned transfer-sets. For each transfer-set, we report the average of normalized entropy of soft-labels.
For both datasets, we observe a transfer-set with higher uncertainty results in more effective KD, and therefore higher validation accuracy for student.}

% \setlength{\textfloatsep}{0.1em}
% \vspace{-0.2cm}
\begin{table}[tb]
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{lcccc}
\hline
dataset  &
\begin{tabular}{@{}c@{}} transfer\\ set \end{tabular}
& $\hat H$ ($\%$) & ERM ($\%$)   & KD ($\%$)\\ \hline \hline

\multirow{3}{*}{CIFAR100}& 
$\mathcal{H}$&
56.4&
52.7&
70.7\\

& $\mathcal{L}$&
5.5&
61.9&
65.3 \\

& $\frac{1}{2}\mathcal{S}$&
0.6&
58.7&
59.2 \\

% & \textit{Z}&
% 58.3 &
% 14.2 $\pm$ 1.2&
% 61.3 $\pm$ 0.6 \\ 
\hline

\multirow{3}{*}{ImageNet}& 
$\mathcal{H}$&
23.1&
65.2&
73.4 \\

& $\mathcal{L}$&
1.8&
65.2&
70.7 \\

& $\frac{1}{2}\mathcal{S}$&
5.9&
62.3&
72.4 \\

% & \textit{Z}&
% 26.7&
% 15.6&
% 58.5 \\
\hline
\end{tabular}
\caption{\new{Effect of the transfer-set's aleatoric uncertainty on student's top-1 validation accuracy. Teacher's accuracy is $74.7\%$ and $76.1\%$ for CIFAR100 and ImageNet, respectively.}}
\label{tab:aleatoric}}
% \vspace{-0.2cm}
\end{table}
% \vspace{-0.2cm}

\noindent\textbf{Observation 2 (Additional Information transfer by Uncertainty Estimation).} \new{Here, we demonstrate the effect the additional information transferred to student from teacher's uncertainty estimation. 
We use the teacher in the above experiment to find $\mathcal{Z} \subset \mathcal{U}$ for which the teacher accuracy is $0\%$ \footnote{$|\mathcal{Z}|$ constitutes $\sim$12$\%$ of the training data for both benchmarks.}.
% Results for training on this zero-accuracy subset  are enclosed in Table~\ref{tab:zero}. 
For samples in $\mathcal{Z}$ the soft-labels generated by the teacher are wrong (i.e., the argmax points to an incorrect class). However, when $\mathcal{Z}$ is used as the transfer-set, the student learns teacher's uncertainty, resulting in surprisingly high validation accuracies as shown in Table~\ref{tab:zero}. This is aligned with our hypothesis that the student best learns teacher's behavior when trained on uncertain data points close to decision boundaries. As seen in Table~\ref{tab:zero}, ERM over $\mathcal{Z}$ results in low generalization accuracy. This can be tied to the fact that labels associated with the dataset are crudely approximated, while using the teachers' outputs allows for capturing the intrinsic aleatoric uncertainties associated with the data.}

\setlength{\textfloatsep}{1pt}
% \vspace{-0.2cm}
\begin{table}[tb]
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{lccccc}
\hline
dataset  &  $\hat H$ ($\%$) & \textit{p} & ERM ($\%$) & KD ($\%$)\\ \hline \hline

CIFAR100& 
58.3&
0.09&
14.2&
61.3\\ \hline

ImageNet&
26.7&
0.14&
15.6&
58.5 \\
\hline
\end{tabular}
% \vspace{-0.2cm}
\caption{\new{Student top-1 validation accuracy when trained using a transfer-set on which the teacher top-1 accuracy is 0$\%$. Here, $p$ denotes the average probability assigned to the ground-truth labels of $\mathcal{Z}$ by the teacher.}}
\label{tab:zero}}
% \vspace{-0.2cm}
\end{table}
% \vspace{-0.2cm}

% \begin{table}[h]
% \RawFloats
% \centering
% \begin{tabular}{lcccc}
%   \hline
% \multirow{2}{*}{transferset} & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{ImageNet} \\ \cline{2-5} 
% & $\hat{H}$ ($\%$)
% & top-1 ($\%$)
% & $\hat{H}$ ($\%$)
% & top-1 ($\%$) \\
%   \hline
%   \hline
% \textit{H}&
% 56.4&
% 70.7 $\pm$ 0.2&
% 23.1&
% 73.4\\

% \textit{L}&
% 5.5&
% 65.3 $\pm$ 0.2&
% 1.8&
% 70.7\\

% $\frac{1}{2}$\textit{S}&
% 0.6&
% 59.2 $\pm$ 0.8&
% 5.9&
% 72.4\\
%   \hline
%   \end{tabular}
%     \caption{\new{Analysis of the correlation between the transferset's aleatoric uncertainty and student generalization accuracy.}
%     \mojan{make sure to get the numbers with the eval.py code}}
%   \label{tab:aleatoric}
% \end{table}

% \noindent\textbf{Evidence 3 (Distribution Uncertainty).} 
% \new{To study the effect of distribution uncertainty, we consider a special case of out-of-distribution data where the images used in KD belong to classes that have never been observed by the teacher during its own training.
% %This ensures that the effect of uncertainty on the student generalization accuracy is isolated from other factors such as image quality, resolution, etc. 
% We divide the classes in each dataset in half to create two disjoint subsets, dubbed $\mathcal{A}$ and $\mathcal{B}$ and the teacher is trained on subset $\mathcal{A}$. Note that in this case both student and teacher classify over half of the classes, i.e., 50 and 500 classes for the CIFAR100  and the ImageNet benchmarks, respectively.}
% % and thus have not seen any data points from the classes in subset \textit{B}. 

% \new{Results are reported in Table~\ref{tab:ood}.
% The validation accuracy of the student trained on the out-of-distribution data ($\mathcal{B}$) is remarkably on par with the student trained on in-distribution data ($\mathcal{A}$). For each case we use the corresponding classes in the validation set to compute the validation accuracies.}
% %In addition, the obtained accuracy on subset \textit{B} is comparable with the accuracy of the ERM baseline. 
% % \mojan{This suggests that a pre-trained teacher together with an arbitrary dataset can replace the original dataset for training a downstream task.}

% % % \setlength{\textfloatsep}{0.1em}
% % % \vspace{-0.2cm}
% % \begin{table}[tb]
% % \resizebox{\columnwidth}{!}{
% % \begin{tabular}{lccccc}
% % \hline
% % \multirow{2}{*}{dataset} & \multirow{2}{*}{T} & \multirow{2}{*}{$\hat H$ ($\%$)} & \multicolumn{2}{c}{teacher top-1 ($\%$)}&
% % \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}student \\ top-1 ($\%$)\end{tabular}}
% % \\ \cline{4-5}
% % &  &  & T & V  &  \\ \hline \hline
% % CIFAR10& 
% % \textit{A}&
% % 0.2&
% % 100&
% % \multirow{2}{*}{98.6}&
% % 98.2 $\pm$ 0.2 \\

% % &\textit{B}&
% % 18.2&
% % % 0.0&
% % -&
% % &
% % 97.5 $\pm$ 0.1 \\ \hline

% % CIFAR100& 
% % \textit{A}&
% % 0.4&
% % 100&
% % \multirow{2}{*}{86.1}&
% % 83.6 $\pm$ 0.6 \\

% % &\textit{B}&
% % 40.3&
% % % 1.9&
% % -&
% % &
% % 82.0 $\pm$ 0.2 \\ \hline

% % ImageNet& 
% % \textit{A}&
% % 3.7&
% % 90.3&
% % \multirow{2}{*}{83.0}&
% % 82.2 \\

% % &\textit{B}&
% % 29.2&
% % % 1.4&
% % -&
% % &
% % 79.6 \\ \hline
% % \end{tabular}
% % \caption{\new{Analysis of distribution uncertainty. Here, T and V denote the transfer and validation sets, respectively. The student validation accuracy trained with ERM on subset \textit{A} is 83.6$\%\pm$0.3 for CIFAR100 and 70.1$\%$ for ImageNet.}}
% % \label{tab:ood}}
% % % \vspace{-0.2cm}
% % \end{table}
% % % \vspace{-0.5cm}

% % \mojan{Pure Gaussian noise provides an extreme case of out-of-distribution data. However, as will be shown in Tab~\ref{tab:qx}, high uncertainty in this scenario implies that the images do not contain the essential features needed for the student to learn.}

% \begin{table}[tb]
% \centering
% \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{lccc}
% \hline
% dataset&
% transfer-set&
% $\hat H$ ($\%$)&
% KD ($\%$)\\ \hline \hline

% \multirow{2}{*}{CIFAR100}& 
% $\mathcal{A}$&
% 0.4&
% 83.6 \\

% & $\mathcal{B}$&
% 40.3&
% 82.0 \\
% \hline

% \multirow{2}{*}{ImageNet}& 
% $\mathcal{A}$&
% 3.7&
% 82.2\\

% & $\mathcal{B}$&
% 3.7&
% 79.6\\

% \hline
% \end{tabular}
% \caption{\new{Analysis of distribution uncertainty.}}
% \label{tab:ood}}
% % \vspace{-0.2cm}
% \end{table}
